Sufficient and Necessary Conditions for Eckart-Young like Result for Tubal Tensors

A valuable feature of the tubal tensor framework is that many familiar constructions from matrix algebra carry over to tensors, including SVD and notions of rank. Importantly, it has been shown that for a specific family of tubal products, an Eckart-Young type theorem holds, i.e., the best low-rank approximation of a tensor under the Frobenius norm is obtained by truncating its tubal SVD. In this paper, we provide a complete characterization of the family of tubal products that yield an Eckart-Young type result. We demonstrate the practical implications of our theoretical findings by conducting experiments with video data and data-driven dynamical systems.

==> macros.tex <==
%% renewals
% \let\oldin\in
% \renewcommand{\in}{\ensuremath{{\oldin}}}
%% util macros
\newcommand{\noun}[1]{\textsc{#1}\xspace}
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\hbs}[1]{\ensuremath{\wh{\bs{#1}}}}
\newcommand{\rank}{\text{\ensuremath{\operatorname{rank}}}}
\newcommand{\argmin}{\text{\ensuremath{\arg\min}}}
\newcommand{\argmax}{\text{\ensuremath{\arg\max}}}
\newcommand{\stt}{\,\,\,\text{s.t.}\,\,\,}
\newcommand{\xx}{\ensuremath{{\times}}}
\newcommand{\code}[1]{\codex{#1}}
\newcommand{\pinv}{\ensuremath{\dagger}}
\renewcommand{\P}{\pinv}
\newcommand{\mpn}{\ensuremath{m \xx p \xx n}}
\newcommand{\pmn}{\ensuremath{p \xx m \xx n}}
\newcommand{\innerprod}[2]{\left\langle #1,#2 \right\rangle }
\newcommand{\mpd}{\ensuremath{m \xx p \xx \ddim}}
\newcommand{\pmd}{\ensuremath{p \xx m \xx \ddim}}
\newcommand{\dimsI}{\ensuremath{I_1 \xx \cdots \xx I_d}}
\newcommand{\dimsr}{\ensuremath{r_1 \xx \cdots \xx r_d}}
\newcommand{\scalemath}[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}
\newcommand{\dbr}[1]{\ensuremath{\llbracket #1 \rrbracket}}

%% tensor notations
\newcommand{\tens}[1]{{\mathcal #1}}
\newcommand{\tA}{\tens{A}}
\newcommand{\tAt}{\tA^{\T}}

\newcommand{\tT}{\tens{T}}


\newcommand{\btA}{\bar{\tens{A}}}
\newcommand{\ttA}{\tilde{\tens{A}}}
\newcommand{\ttAt}{\ttA^{\T}}
\newcommand{\thA}{\widehat{\tA}}
\newcommand{\tthA}{\widehat{\ttA}}
\newcommand{\thAt}{\thA^{\T}}
\newcommand{\tthAt}{\tthA^{\T}}
\newcommand{\tB}{\tens{B}}
\newcommand{\tBt}{\tB^{\T}}
\newcommand{\thB}{\widehat{\tB}}
\newcommand{\thBt}{\thB^{\T}}
\newcommand{\tR}{\tens{R}}
\newcommand{\thR}{\widehat{\tR}}
\newcommand{\tRt}{\tR^{\T}}
\newcommand{\tM}{\tens{M}}
\newcommand{\thM}{\widehat{\tM}}
\newcommand{\tMt}{\tM^{\T}}

\newcommand{\tV}{\tens{V}}
\newcommand{\tVt}{\tV^{\T}}
\newcommand{\tVH}{\tV^{\H}}
\newcommand{\thV}{\widehat{\tV}}
\newcommand{\thVt}{\thV^{\T}}
\newcommand{\tU}{\tens{U}}
\newcommand{\tUt}{\tU^{\T}}
\newcommand{\thU}{\widehat{\tU}}
\newcommand{\thUt}{\thU^{\T}}
\newcommand{\tX}{\tens{X}}
\newcommand{\thX}{\widehat{\tX}}
\newcommand{\tY}{\tens{Y}}
\newcommand{\tYt}{\tY^{\T}}
\newcommand{\thY}{\widehat{\tY}}
\newcommand{\thYt}{\thY^{\T}}

\newcommand{\qprm}{q^{\prime}}

\newcommand{\tS}{\tens{S}}
\newcommand{\tSt}{\tS^{\T}}
\newcommand{\thS}{\widehat{\tS}}
\newcommand{\thSt}{\thS^{\T}}
\newcommand{\teJ}{\tens{J}}
\newcommand{\theJ}{\widehat{\teJ}}
\newcommand{\tI}{\tens{I}}
\newcommand{\thI}{\widehat{\tI}}
\newcommand{\tC}{\tens{C}}
\newcommand{\tCt}{\tC^{\T}}
\newcommand{\thC}{\widehat{\tC}}
\newcommand{\thCt}{\thC^{\T}}
\newcommand{\tG}{\tens{G}}
\newcommand{\tGt}{\tG^{\T}}
\newcommand{\thG}{\widehat{\tG}}

\newcommand{\tVe}{\tV_{\epsilon}}
\newcommand{\tVet}{\tVe^{\T}}
\newcommand{\thVe}{\widehat{\tV}_\epsilon}
\newcommand{\thVet}{\thVe^{\T}}
\newcommand{\tUe}{\tU_{\epsilon}}
\newcommand{\tUet}{\tUe^{\T}}
\newcommand{\thUe}{\widehat{\tU}_\epsilon}
\newcommand{\thUet}{\thUe^{\T}}
\newcommand{\tSe}{\tS_{\epsilon}}
\newcommand{\tSet}{\tSe^{\T}}
\newcommand{\thSe}{\widehat{\tS}_{\epsilon}}
\newcommand{\thSet}{\thSe^{\T}}

\newcommand{\tCe}{\tC_{\epsilon}}
\newcommand{\tCet}{\tCe^{\T}}
\newcommand{\thCe}{\widehat{\tC}_\epsilon}
\newcommand{\thCet}{\thCe^{\T}}

\newcommand{\tE}{\tens{E}}
\newcommand{\thE}{\widehat{\tE}}
\newcommand{\tQ}{\tens{Q}}
\newcommand{\tQt}{\tQ^{\T}}
\newcommand{\tQh}{\tQ^{\H}}
\newcommand{\thQ}{\widehat{\tQ}}
\newcommand{\thQt}{\thQ^{\T}}
\newcommand{\hsigma}{\ensuremath{\hat{\sigma}}}
\newcommand{\tZ}{\tens{Z}}
\newcommand{\tZt}{\tZ^{\T}}
\newcommand{\thZ}{\widehat{\tZ}}
\newcommand{\thZt}{\thZ^{\T}}

\newcommand{\tW}{\tens{W}}
\newcommand{\tWt}{\tW^{\T}}
\newcommand{\thW}{\widehat{\tW}}
\newcommand{\thWt}{\thW^{\T}}

\newcommand{\tP}{\tens{P}}
\newcommand{\tPt}{\tP^{\T}}
\newcommand{\thP}{\widehat{\tP}}
\newcommand{\thPt}{\thP^{\T}}

\newcommand{\tH}{\tens{H}}
\newcommand{\tHt}{\tH^{\T}}
\newcommand{\thH}{\widehat{\tH}}
\newcommand{\thHt}{\thH^{\T}}

\newcommand{\upbb}[2]{\ensuremath{{#1}^{(#2)}}}

\newcommand{\tWh}{\upbb{\tW}{h}}
\newcommand{\tWht}{( \tWh )^{\T}}
\newcommand{\thWh}{\widehat{\upbb{\tW}{h}}}
\newcommand{\thWht}{(\thWh)^{\T}}

\newcommand{\tCh}{\upbb{\tC}{h}}
\newcommand{\tCht}{(\tCh)^{\T}}
\newcommand{\thCh}{\widehat{\upbb{\tC}{h}}}
\newcommand{\thCht}{(\thCh)^{\T}}


\newcommand{\tWl}{\upbb{\tW, \ell}}
\newcommand{\tWlt}{( \tWh )^{\T}}
\newcommand{\thWl}{\widehat{\upbb{\tW}{\ell}}}
\newcommand{\thWlt}{(\thWh)^{\T}}

\newcommand{\tCl}{\upbb{\tC}{\ell}}
\newcommand{\tClt}{(\tCh)^{\T}}
\newcommand{\thCl}{\widehat{\upbb{\tC}{\ell}}}
\newcommand{\thClt}{(\thCh)^{\T}}


\newcommand{\qb}{Q_{\tB}}
\newcommand{\qv}{Q_{\tV}}
\newcommand{\pb}{P_{\tB}}
\newcommand{\tpb}{\tilde{P}_{\tB}}
\newcommand{\pv}{P_{\tV}}
\newcommand{\rbb}{R_{\matb}}
\newcommand{\rvv}{R_{\matr}}






%% matrix notations
\newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\matA}{\mat{A}}
\newcommand{\matX}{\mat{X}}
\newcommand{\matR}{\mat{R}}
\newcommand{\matRt}{\matR^\T}
\newcommand{\matQ}{\mat{Q}}
\newcommand{\matE}{\mat{E}}
\newcommand{\matQt}{\matQ^{\T}}

\newcommand{\matQip}{\ensuremath{{\matQ_i}_\perp}}
\newcommand{\matQipt}{\ensuremath{\matQip^\T}}

\newcommand{\matP}{\mat{P}}
\newcommand{\matPt}{\matP^{\T}}
\newcommand{\mattP}{\tilde{\mat{P}}}
\newcommand{\mattPt}{\mattP^{\T}}
\newcommand{\matXt}{\matX^{\T}}
\newcommand{\matAt}{\matA^{\T}}
\newcommand{\bmatA}{\bar{\matA}}
\newcommand{\bmatAt}{\bmatA^{\T}}
\newcommand{\mata}{\mat{a}}
\newcommand{\matV}{\mat{V}}
\newcommand{\matVt}{\ensuremath{\matV^{\T}}}
\newcommand{\matU}{\mat{U}}
\newcommand{\matUt}{\matU^{\T}}
\newcommand{\matS}{\mat{S}}
\newcommand{\matSt}{\ensuremath{\matS^{\T}}}
\newcommand{\matT}{\mat{T}}
\newcommand{\matTt}{\ensuremath{\matT^{\T}}}
\newcommand{\mats}{\mat{s}}
\newcommand{\hmats}{\hat{\mats}}
\newcommand{\matr}{\mat{r}}
\newcommand{\maty}{\mat{y}}
\newcommand{\amatr}{\vec{\matr}}
\newcommand{\matC}{\mat{C}}
\newcommand{\matCt}{\matC^{\T}}

\newcommand{\matAr}{\mat{A}_r}


\newcommand{\matD}{\mat{D}}
\newcommand{\matd}{\mat{d}}
\newcommand{\matds}[1]{\matd^{(#1)}}
\newcommand{\ddi}{\matds{i}}
\newcommand{\ddim}{\ensuremath{D^{\xx}}}

\newcommand{\matG}{\mat{G}}
\newcommand{\matGt}{\ensuremath{\matG^{\T}}}

\newcommand{\matZ}{\mat{Z}}
\newcommand{\matZt}{\matZ^{\T}}
\newcommand{\matY}{\mat{Y}}
\newcommand{\matYt}{\matY^{\T}}

\newcommand{\matH}{\mat{H}}
\newcommand{\matHt}{\matH^\T}

\newcommand{\matSigma}{\boldsymbol{\Sigma}}
\newcommand{\matOmega}{\boldsymbol{\Omega}}
\newcommand{\matOmegat}{\matOmega^\T}
\newcommand{\matPsi}{\boldsymbol{\Psi}}
\newcommand{\matPsit}{\matPsi^\T}

\newcommand{\matpi}{\boldsymbol{\pi}}
\newcommand{\matpit}{\matpi^\T}

\newcommand{\matK}{\mat{K}}
\newcommand{\matM}{\mathbf{M}}
\newcommand{\matMi}{\matM^{-1}}
\newcommand{\matMt}{\matM^{\T}}
\newcommand{\matW}{\mathbf{W}}
\newcommand{\matWt}{\matW^{\T}}
\newcommand{\T}{\mat{T}}
\newcommand{\CT}{\mat{H}}
\newcommand{\bell}{{(\ell)}}

\newcommand*\wh[1]{\widehat{#1}}
\newcommand*\wt[1]{\widetilde{#1}}
%% vector notations
\renewcommand{\u}{\mat{u}}
\newcommand{\ut}{\ensuremath{\u^{\T}}}
\newcommand{\hu}{\ensuremath{\hat{\u}}}
\renewcommand{\v}{\mat{v}}
\newcommand{\hv}{\ensuremath{\hat{\v}}}
\newcommand{\rrho}{\ensuremath{\bs{\rho}}}
\newcommand{\eeta}{\ensuremath{\bs{\eta}}}
\newcommand{\pphi}{\ensuremath{\bs{\varphi}}}
\newcommand{\rb}{\mat{r}}
\newcommand{\w}{\mat{w}}
% \newcommand{\wt}{\ensuremath{\w^{\T}}}
\renewcommand{\b}{\mat{b}}
\newcommand{\bt}{\ensuremath{\b^{\T}}}
\newcommand{\x}{\mat{x}}
\newcommand{\h}{\mat{h}}
\newcommand{\g}{\mat{g}}
\newcommand{\e}{\mat{e}}
\newcommand{\xt}{\x^{\T}}
\newcommand{\gt}{\g^{\T}}
% \newcommand{\v}{\mat{v}}
\newcommand{\vt}{\v^{\T}}
\newcommand{\q}{\mat{q}}
\newcommand{\qt}{\q^{\T}}
\newcommand{\p}{\mat{p}}
\newcommand{\y}{\mat{y}}
\newcommand{\bmaty}{\bar{\y}}
\newcommand{\bmatx}{\bar{\x}}
\newcommand{\z}{\mat{z}}
% \newcommand{\aa}{\mat{aa}}
\newcommand{\matB}{\mat{B}}
\newcommand{\matI}{\mat{I}}
\newcommand{\matF}{\mat{F}}
\newcommand{\matFt}{\matF^{\T}}
\newcommand{\matBt}{\matB^{\T}}
\newcommand{\si}{\ensuremath{^{(i)}}}
\newcommand{\vpsi}{\boldsymbol{\psi}}
\newcommand{\vtau}{\boldsymbol{\tau}}
\newcommand{\vepsilon}{\boldsymbol{\epsilon}}
\newcommand{\vmu}{\boldsymbol{\mu}}
\newcommand{\vom}{\boldsymbol{\omega}}
\newcommand{\matGamma}{\boldsymbol{\Gamma}}
\newcommand{\TT}{\mathcal{T}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\HH}{\mathcal{H}}
\newcommand{\FF}{\mathcal{F}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\LT}{{\LL^2}}

% \newcommand{\qb}{Q_{\tB}}
% \newcommand{\qv}{Q_{\tV}}
\newcommand{\ovec}{\operatorname{vec}}
\newcommand{\reshape}{\operatorname{reshape}}



\newcommand{\matb}{\mat{b}}
\newcommand{\matbt}{\matb^{\T}}
\newcommand{\mate}{\mat{e}}
\newcommand{\matet}{\mate^{\T}}
\newcommand{\matXi}{\boldsymbol{\Xi}}

\newcommand{\bsc}{\bs{c}}
\newcommand{\bsct}{\bsc^{\T}}

\newcommand{\tlX}{\tilde{X}}
\newcommand{\tlY}{\tilde{Y}}

%% field notations
\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\FFF}{\mathbb{F}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\sgnErr}{E_{SGN}}
\newcommand{\tsgnErr}{\tE_{SGN}}
\newcommand{\Ei}{E^{(i)}}
\newcommand{\spacex}{\boldsymbol{\mathcal{X}}}
\newcommand{\spacey}{\boldsymbol{\mathcal{Y}}}

%% norms
\newcommand{\dotp}[1]{\langle #1 \rangle}
\newcommand{\dotps}[1]{\dotp{#1}^2}
\newcommand{\FDot}[1]{\dotp{#1}_{F}}
\newcommand{\FDotS}[1]{\dotps{#1}_{F}}
\newcommand{\LTdotp}[1]{\dotp{#1}_{\LL^2}}
\newcommand{\LTdotps}[1]{\LTdotp{#1}^2}

\newcommand{\HNorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
\newcommand{\HNormS}[1]{\HNorm{#1}}

\newcommand{\TNorm}[1]{\|#1\|_{2}}
\newcommand{\TNormS}[1]{\TNorm{#1}^2}
\newcommand{\GNorm}[1]{\|#1\|}
\newcommand{\GNormS}[1]{\GNorm{#1}^2}
\newcommand{\GNormd}[1]{\left\|#1\right\|}
\newcommand{\GNormSd}[1]{\GNormd{#1}^2}
\newcommand{\FNorm}[1]{\|#1\|_{F}}
\newcommand{\FNormS}[1]{\FNorm{#1}^2}
\newcommand{\FNormd}[1]{\lVert#1\rVert_{F}}
\newcommand{\FNormSd}[1]{\FNormd{#1}^2}
\newcommand{\NNorm}[1]{\|#1\|_{*}}

\newcommand{\LTNorm}[1]{\|#1\|_{\LT}}
\newcommand{\LTNormS}[1]{\LTNorm{#1}^2}

\newcommand{\tNorm}[1]{\|#1\|_{top}}
\newcommand{\tNormS}[1]{\tNorm{#1}^2}

\newcommand{\war}[1]{\ensuremath{\overrightarrow{\vphantom{A}{#1}}}}
\newcommand{\bwar}[1]{\war{\bs{#1}}}

\newcommand{\trc}{\ensuremath{\operatorname{Tr}}}
\newcommand{\trace}[1]{\ensuremath{\operatorname{Tr}\left(#1 \right)}}
\newcommand{\ftr}[1]{\ensuremath{\operatorname{f-Tr}(#1)}}

%% transforms and decompositions
\newcommand{\clr}{\noun{clr}}
\newcommand{\rclr}{\noun{rclr}}
\newcommand{\tsvdm}{\textsc{tsvdm}\xspace}
\newcommand{\tcam}{\textsc{tcam}\xspace}
\newcommand{\tca}{\textsc{tca}\xspace}
\newcommand{\tsvdmii}{\ensuremath{t}-\textsc{svdmii}\xspace}

%% tensor operations
\newcommand{\calf}{{\cal F}}
\newcommand{\mx}[1]{\ensuremath{\times_{#1}}}
\newcommand{\tsub}[1]{\ensuremath{\times_{#1}}}
\newcommand{\tsM}{\ensuremath{\tsub{3}\matM}}
\newcommand{\tsMinv}{\ensuremath{\tsub{3}\matM^{-1}}}
\newcommand{\ttprod}[1]{{\star}_{{\scriptscriptstyle{\hspace{-0.5pt}#1}\hspace{0.5pt} }}}
\newcommand{\Mprod}{\ttprod{\matM}}
\newcommand{\mm}{\ttprod{\matM}}
\newcommand{\mmz}{\ttprod{\matM_0}}
\newcommand{\mmo}{\ttprod{\matM_1}}
% \newcommand{\ff}{\tprod{\mathcal{F}}}
\newcommand{\ff}{\ttprod{{F}}}
\newcommand{\pp}{\ttprod{{\Phi}}}
\newcommand{\muni}{\ensuremath{\Mprod{\textnormal{-unitary}}}\xspace}
\newcommand{\morth}{\ensuremath{\Mprod{\textnormal{-orthogonal}}}\xspace}
\newcommand{\pmorth}{\ensuremath{\textnormal{pseudo }\Mprod{\textnormal{-orthogonal}}}\xspace}
\newcommand{\Pmorth}{\ensuremath{\textnormal{Pseudo }\Mprod{\textnormal{-orthogonal}}}\xspace}
\newcommand{\rnk}{\ensuremath{\operatorname{rank}}}
\newcommand{\trnk}[1]{t\operatorname{-}\rnk_{#1} }
\newcommand{\Npr}{\ensuremath{N^{\prime}}}
\newcommand{\unf}[2]{\ensuremath{{#1}_{(#2)}} }
\newcommand{\supl}[1]{\ensuremath{{#1}^{[\ell]}} }
\newcommand{\fld}[2]{\ensuremath{\operatorname{fold}({#1}, #2)}}
\newcommand{\bxx}{\smash{{\setlength{\fboxsep}{0pt}\raisebox{-.5pt}{\scalebox{1.5}{\ensuremath{\xx\vphantom{A}}}}\hspace{-1pt}}}{}}

\newcommand{\bcirc}{\mathtt{bcirc}}
\newcommand{\fold}{\operatorname{fold}}


% \newcommand{\XX}{\mathbin{\tikz [x=1.6ex,y=1.6ex,line width=.2ex] \draw(0.5,0)-- (1.5,1) (0.5,1) -- (1.5,0);}}
\newcommand{\XX}{\hspace*{1pt}{\textstyle\bigtimes}}

\newcommand{\OX}{{\textstyle \bigotimes}}
%% general macros
\newcommand{\Mpinv}{\mathbf{+}}
\newcommand{\mmpinv}{\ensuremath{\Mprod}\textnormal{-pseudo inverse}\xspace}

% multilinear algebra
\newcommand{\fM}{\ensuremath{\mathfrak{M}} }

%% algorithmic
\algnewcommand{\IfThenElse}[3]{% \IfThenElse{<if>}{<then>}{<else>}
	\State \algorithmicif\ #1\ \algorithmicthen\ #2\ \algorithmicelse\ #3}
\algnewcommand\Input{\item[\textbf{Input:}]}%
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\INPUT{\item[\algorithmicinput]}

\algnewcommand\Noln{\item[\hspace{28pt}]}%
\algnewcommand\algorithmicnoln{\hspace{28pt}}
\algnewcommand\NOLN{\item[\algorithmicnoln]}

\algnewcommand\SState{\State \hskip-1.em }
\algnewcommand\algorithmicswitch{\textbf{switch}}
\algnewcommand\algorithmiccase{\textbf{case}}
\algnewcommand\algorithmicassert{\texttt{assert}}
\algnewcommand\Assert[1]{\State \algorithmicassert(#1)}

\algnewcommand\Output{\item[\textbf{Output:}]}%
% \algnewcommand\algorithmicinput{\textbf{Input:}}

\algnewcommand\Params{\item[\textbf{Parameters:}]}%
\algnewcommand\algorithmicparams{\textbf{Parameters:}}
\algnewcommand\PARAMS{\item[\algorithmicparams]}

\algnewcommand\Outputline{\item[]}%
%% text abbvs 
\newcommand{\samplemode}{\emph{sample mode} }
\newcommand{\featuremode}{\emph{feature mode} }
\newcommand{\omx}{{\it omics} }
\newcommand{\LFB}{LFB }
\newcommand{\DFB}{DFB}
\newcommand{\supp}[1]{\ensuremath{\operatorname{supp}\{#1\}}}

\newcommand{\sigmaset}{{\scalebox{1.4}{$\upsigma$}}}
% todo macros
% \newcommandx{\unsure}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
% \newcommandx{\change}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
% \newcommandx{\info}[2][1=]{\todo[linecolor=OliveGreen,backgroundcolor=OliveGreen!25,bordercolor=OliveGreen,#1]{#2}}
% \newcommandx{\improvement}[2][1=]{\todo[linecolor=Plum,backgroundcolor=Plum!25,bordercolor=Plum,#1]{#2}}
% \newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}

% \newcommand{\COMMENTFILE}{child_docs/commentfile.tex}
% \newcommand{\ecomment}[2]{\unsure{{\bf (line \number\inputlineno,#1,#2)}:\newline%
								% 	\ExecuteMetaData[\COMMENTFILE]{#1}}\xspace}
% \ExecuteMetaData[child_docs/commentfile.tex]


%% FIGURES
% pbx panel
\newcommand{\pbxstd}{Fig.1b\xspace}
\newcommand{\pbxtca}{Fig.1c\xspace}
\newcommand{\pbxfunnel}{Fig.1d\xspace}
\newcommand{\pbxbars}{Fig.1e\xspace}

% fibers panel
\newcommand{\fibersctf}{Fig.fb\xspace}
\newcommand{\fiberstca}{Fig.1g\xspace}
\newcommand{\fibersfunnel}{Fig.1h\xspace}
\newcommand{\fiberstimeseries}{Fig.1i\xspace}
\newcommand{\fibersheatmap}{Fig.1j\xspace}

% ibd (main) panel
\newcommand{\ibdrocs}{Fig.2a\xspace}
\newcommand{\ibdloadings}{Fig.2b\xspace}
\newcommand{\ibdtca}{Fig.2c\xspace}
\newcommand{\ibdtimeseries}{Fig.2d\xspace}

% Snyder panel
\newcommand{\snydertca}{Fig.2e\xspace}
\newcommand{\snyderheatmap}{Fig.2f\xspace}

%% Annotations
\newcommand{\Uria}[1]{\textcolor{blue}{[Uria: #1]}}
\newcommand{\Haim}[1]{\textcolor{red}{[Haim: #1]}}

%% colors
\definecolor{PinkC}{HTML}{ff66ff}
\definecolor{GreenC}{HTML}{33cc33}
\definecolor{BlueC}{HTML}{0099ff}
\definecolor{PurpleC}{HTML}{cc00cc}

\newcommand{\cpink}[1]{\textcolor{PinkC}{#1}}
\newcommand{\cgreen}[1]{\textcolor{GreenC}{#1}}
\newcommand{\cblue}[1]{\textcolor{BlueC}{#1}}
\newcommand{\cpurple}[1]{\textcolor{PurpleC}{#1}}

\newcommand{\matMs}{\ensuremath{\matM}^*}
\newcommand{\YY}{\ensuremath{\mathbb{Y}}}
\newcommand{\hYY}{\ensuremath{\widehat{\mathbb{Y}}}}
\newcommand{\YYr}{\ensuremath{\YY_r}}
\newcommand{\hYYr}{\ensuremath{\hYY_r}}

\newcommand{\spc}{\ensuremath{\texttt{spec}}}
\newcommand{\wc}{\ensuremath{\rightharpoonup}}

\newcommand{\doublecref}[2]{%
  \hyperref[#2]{\namecref{#1}~\labelcref*{#1}~\ref*{#2}}%
}
% \newcommand{\doubleCref}[2]{%
%   \hyperref[#2]{\nameCref{#1}~\labelcref*{#1}~\Cref{#2}}%
% }
\newcommand{\doubleCref}[2]{%
  \hyperref[#2]{\labelcref*{#1}~\Cref{#2}}%
}
\newcommand{\ccreff}[2]{%
  \hyperref[#2]{\Cref{#2}(\labelcref*{#1})}%
}



\newif\ifuriaread % create a new conditional
\uriareadfalse % set it to false
\newcommand{\ureminder}[1]{%
    \Uria{%
        Set \textbackslash{}uriaread to false if you want to remove this reminder.\newline%
        #1%
    }}
\newcommand{\urif}[1]{%
    \ifuriaread%
        \ureminder{#1}%
    \else%
    \fi}




% \newcommand{\alg}[1]{\ensuremath{\eufm{#1}} }
% \newcommand{\alg}[1]{\ensuremath{\mathbbb{#1}} }
\newcommand{\alg}[1]{\ensuremath{\mathcal{#1}} }
\newcommand{\TA}{\alg{A}}
\newcommand{\TB}{\alg{B}}
\newcommand{\TM}{\alg{M}}
\newcommand{\TE}{\alg{E}}
\newcommand{\FT}{\alg{T}}
\newcommand{\FQ}{\alg{Q}}
\newcommand{\FR}{\alg{R}}

\newcommand{\ellinf}{\ell_\infty}
\newcommand{\elltwo}{\ell_2}

\newcommand{\hspc}[1]{\ensuremath{\boldsymbol{ #1}}}
% \newcommand{\hspc}[1]{\ensuremath{\boldsymbol{\EuScript #1}}}
% \newcommand{\cH}{\ensuremath{{\hspc H}}}
\newcommand{\cH}{\ensuremath{{\alg H}}}
\newcommand{\cE}{\ensuremath{{\hspc E}}}
\newcommand{\chH}{\ensuremath{\widehat{\cH}}}
\newcommand{\chHp}{\ensuremath{\widehat{\cH}^p}}

\newcommand{\cX}{\ensuremath{{\hspc X}}}

\newcommand{\cB}{\ensuremath{{\hspc B}}}
\newcommand{\chB}{\ensuremath{\widehat{\cB}}}
\newcommand{\chBp}{\chB^p}
\newcommand{\chBpd}{(\chB^p)^*}
\newcommand{\fphi}{\FF_{\bs{\varphi}}}
\newcommand{\fphis}{{\fphi}^*}

% \newcommand{\cHs}{\ensuremath{\cH^{*}}}
% \newcommand{\chHs}{\ensuremath{{\chH}^*}}
\newcommand{\hhat}[1]{\hat{\hspace{-1pt}{#1}}}
\newcommand{\dotmp}[1]{\left\llangle #1 \right\rrangle}
\newcommand{\dotph}[1]{\dotp{#1}_{\cH}}
\newcommand{\dotphh}[1]{\dotp{#1}_{\chH}}
\newcommand{\dotphhp}[1]{\dotp{#1}_{\chH^p}}
% \newcommand{\dotphs}[1]{\dotph{#1}^2}
\newcommand{\mpT}{\ensuremath{m \xx p \xx {\hspc T}}}
\newcommand{\mpzo}{\ensuremath{m \xx p \xx [0,1]}}
\newcommand{\cHNorm}[1]{\GNorm{#1}_{\cH}}
\newcommand{\cHNormS}[1]{\cHNorm{#1}^2}
\newcommand{\cHsNorm}[1]{\GNorm{#1}_{\cHs}}
\newcommand{\cHsNormS}[1]{\cHsNorm{#1}^2}
\newcommand{\cHsNormd}[1]{\GNormd{#1}_{\cHs}}
\newcommand{\cHsNormSd}[1]{\cHsNormd{#1}^2}

\newcommand{\dotpx}[1]{\dotp{#1}_{\cX}}
\newcommand{\cXNorm}[1]{\GNorm{#1}_{\cX}}
\newcommand{\cXNormS}[1]{\cXNorm{#1}^2}

\newcommand{\HSNorm}[1]{\GNorm{#1}_{\operatorname{HS}}}
\newcommand{\HSNormS}[1]{\HSNorm{#1}^2}
\newcommand{\dotphs}[1]{\dotp{#1}_{\operatorname{HS}}}

\newcommand{\Blt}{\ensuremath{{\hspc B}(\ell_2)}}
\newcommand{\BltNorm}[1]{\GNorm{#1}_{\Blt}}
\newcommand{\BltNormS}[1]{\BltNorm{#1}^2}


\newcommand{\ltNorm}[1]{\GNorm{#1}_{\ell_2}}
\newcommand{\ltNormS}[1]{\ltNorm{#1}^2}
\newcommand{\dotplt}[1]{\dotp{#1}_{\ell_2}}

\newcommand{\cY}{\ensuremath{{\hspc Y}}}
\newcommand{\cYd}{\cY^*}
\newcommand{\cYNorm}[1]{\GNorm{#1}_{\cY}}
\newcommand{\cYNormS}[1]{\cYNorm{#1}^2}

\newcommand{\cYp}{\cY'}
\newcommand{\cYpNorm}[1]{\GNorm{#1}_{\cYp}}
\newcommand{\cYpNormS}[1]{\cYpNorm{#1}^2}

\newcommand{\infNorm}[1]{\GNorm{#1}_{\infty}}
\newcommand{\infNormS}[1]{\infNorm{#1}^2}

\newcommand{\chHNorm}[1]{\GNorm{#1}_{\chH}}
\newcommand{\chHNormS}[1]{\chHNorm{#1}^2}

\newcommand{\chHpNorm}[1]{\GNorm{#1}_{\chHp}}
\newcommand{\chHpNormS}[1]{\chHpNorm{#1}^2}

\newcommand{\op}{\ensuremath{{\operatorname{op}}}}

\newcommand{\opNorm}[1]{\GNorm{#1}_{\op}}
\newcommand{\opNormS}[1]{\opNorm{#1}^2}
\newcommand{\opNormd}[1]{\GNormd{#1}_{\op}}
\newcommand{\opNormSd}[1]{\opNormd{#1}^2}

\newcommand{\ropNorm}[1]{\GNorm{#1}_{\FFF{-}\op}}
\newcommand{\ropNormS}[1]{\ropNorm{#1}^2}

\newcommand{\cHopNorm}[1]{\GNorm{#1}_{\cH{-}\op}}
\newcommand{\cHopNormS}[1]{\cHopNorm{#1}^2}

\newcommand{\fqopNorm}[1]{\GNorm{#1}_{\FQ{-}\op}}
\newcommand{\fqopNormS}[1]{\fqopNorm{#1}^2}


\newcommand{\cali}{\ensuremath{\hspc I}}

\newcommand{\cPo}{\ensuremath{{\hspc P}_1}}
\newcommand{\cHz}{\ensuremath{{\hspc H}_0}}
\newcommand{\cHo}{\ensuremath{{\hspc H}_1}}
\newcommand{\cHs}{\cH_{*}}
\newcommand{\cHsn}{\cH_{\divideontimes}}
\newcommand{\cHsq}[1]{\cH_{*^{#1}}}

\newcommand{\calfi}{\ensuremath{{\calf}^{-1}}}


\renewcommand{\Re}[1]{\operatorname{Re}(#1)}
\renewcommand{\Im}[1]{\operatorname{Im}(#1)}

\newcommand{\Hom}{\operatorname{Hom}}
\newcommand{\Aut}{\operatorname{Aut}}
\newcommand{\var}{\mathtt{var}}
\newcommand{\cov}{\mathtt{cov}}
\newcommand{\cor}{\mathtt{cor}}
\newcommand{\mean}{\mathtt{mean}}

\newcommand{\fqp}{\FQ^p}
\newcommand{\chp}{\cH^p}
\newcommand{\qrnk}{\ensuremath{\FQ\operatorname{{-}rank}}}

\newcommand{\fqmpNorm}[1]{\GNorm{#1}_{\FQ^{m \xx p}}}
\newcommand{\fqmpNormS}[1]{\GNormS{#1}_{\FQ^{m \xx p}}}

\newcommand{\diag}{\operatorname{diag}}

\newcommand{\fp}{{\vartriangle}}
\newcommand{\Ehm}{\wh{\matE}^{(m)}}
\newcommand{\Ehp}{\wh{\matE}^{(p)}}
\newcommand{\ehpe}{\wh{e}^{(p)}}

